MiPa: Mixed Patch Infrared-Visible Modality Agnostic Object Detection

In real-world scenarios, using multiple modalities like visible (RGB) and infrared (IR) can greatly improve the performance of a predictive task such as object detection (OD). Multimodal learning is a common way to leverage these modalities, where multiple modality-specific encoders and a fusion module are used to improve performance. In this paper, we tackle a different way to employ RGB and IR modalities, where only one modality or the other is observed by a single shared vision encoder. This realistic setting requires a lower memory footprint and is more suitable for applications such as autonomous driving and surveillance, which commonly rely on RGB and IR data. However, when learning a single encoder on multiple modalities, one modality can dominate the other, producing uneven recognition results. This work investigates how to efficiently leverage RGB and IR modalities to train a common transformer-based OD vision encoder, while countering the effects of modality imbalance. For this, we introduce a novel training technique to Mix Patches (MiPa) from the two modalities, in conjunction with a patch-wise modality agnostic module, for learning a common representation of both modalities. Our experiments show that MiPa can learn a representation to reach competitive results on traditional RGB/IR benchmarks while only requiring a single modality during inference. Our code is available at: https://github.com/heitorrapela/MiPa.

==> backup.tex <==
\begin{table}[!htp]
    
    \caption{Comparison of detection performance over different baselines and MiPa for DINO ConvNeXt in LLVIP and FLIR datasets. The evaluation is done for RGB, Thermal, and the average of the modalities.}
    \centering
    \resizebox{1.0\columnwidth}{!}{%
    \begin{tabular}{qgggggggggggggg}
    \toprule
   \rowcolor{white}
    {} & \multicolumn{3}{c}{\textbf{Dataset: LLVIP} (\textbf{AP$_{50}\uparrow$} )} \\
    
    \cmidrule(lr){2-4}
    \addlinespace[5pt]
            
    \cellcolor[HTML]{FFFFFF} \multirow{1}{*}[+0.9em]{\textbf{Modality}} &  \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{RGB}} & \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{Thermal}} & \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{Average}}   \\
    

        
        \midrule

       \rowcolor{white}
        RGB & 90.77 ± 0.34 &	92.20 ± 0.62 & 91.48 \\																																
        THERMAL & 63.23 ± 9.02  &	95.60 ± 0.45 & 79.42  \\		

        
        \rowcolor{white}
        BOTH [$\rho=0.25$] & 76.70 ± 4.04 & 96.27 ± 0.48  &	86.48 \\
        
        BOTH [$\rho=0.50$] & 81.40 ± 2.55 & 95.50 ± 0.57  &	88.45 \\				
        
        \rowcolor{white}
        BOTH [$\rho=0.75$]   & 79.80 ± 1.49 & 95.60 ± 0.57  &	87.70 \\		
        
        \cmidrule(lr){1-11}
        \textbf{MiPa (Ours)} &  81.03 ± 0.74 & 96.43 ± 0.12  &	88.73 \\	
        

	\midrule		

        
        \rowcolor{white}
        {} & \multicolumn{3}{c}{\textbf{Dataset: FLIR} (\textbf{AP$_{50}\uparrow$} )} \\
        
        \cmidrule(lr){2-4}
        \addlinespace[5pt]
                
        \cellcolor[HTML]{FFFFFF} \multirow{1}{*}[+0.9em]{\textbf{Modality}} &  \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{RGB}} & \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{Thermal}} & \cellcolor[HTML]{FFFFFF}\multirow{2}{*}[1em]{\textbf{Average}}   \\
        											
     
    \midrule
       \rowcolor{white}
        RGB & 52.77 ± 1.43 &	48.33 ± 1.87 &	50.55  \\	

        THERMAL & 39.43 ± 0.39 & 58.87 ± 0.87 & 49.15 \\																						
        \rowcolor{white}
        BOTH [$\rho=0.25$]  & 45.87 ± 1.14  & 54.53 ± 1.20 &	50.20  \\																	
        BOTH [$\rho=0.50$]  & 48.00 ± 2.87 & 55.40 ± 0.05 &	51.70 \\																			
        \rowcolor{white}
        BOTH [$\rho=0.75$]  & 52.97 ± 3.03 & 57.53 ± 0.86 &	55.25  \\																	
        
        \midrule
        \textbf{MiPa (Ours)} & 46.17 ± 0.66 &	56.27 ± 0.33  &	51.22  \\																				
        

        
        
        
        
								


        
                

        

        
        
        
    											



        
        
        
        


        
        
        
       

           					
        
    \bottomrule
   
        
    \end{tabular}
    }

\label{tab:tab0_convnext}
\end{table}





\noindent The MiPa method is compatible with any patch-based feature extractor: which could be either a Transformer or a CNN. Nevertheless, the technique should work best alongside Transformer-based models. The transformer is made with a Self-Attention module, while the CNN has a convolutional layer. 
In the Self-Attention module, every patch contains the same channels, while in the patch-based convolution layer, the different neighboring patches go through their respective convolution kernel. In the case of the Self-Attention, the full approximation of $I$ is fed to it:
\[SA(I_a + \eta),\]
But for the convolution kernels, fractions of $I_a$ corresponding to each kernel are sent to each of them, such as in the following:
\[I_a = I_{a1} + I_{a2} + ... + I_{ak} + \eta\]
\[C_i(I_ai + \eta)\]
Consequently, each kernel gets a poorer/inferior approximation of $I$. To verify that hypothesis, we are comparing the results from the pure MiPa in conjunction with ConvNeXt versus SWIN. Though MiPa ConvNeXt is expected to be outperformed by SWIN, the next section will detail how the Modality Agnostic module helps decrease the performance gap between the modalities.

